XL-Sum: Large-Scale Multilingual Abstractive Summarization for 44 Languages

Contemporary works on abstractive text summarization have focused primarily on high-resource languages like English, mostly due to the limited availability of datasets for low/mid-resource ones. In this work, we present XL-Sum, a comprehensive and diverse dataset comprising 1 million professionally annotated article-summary pairs from BBC, extracted using a set of carefully designed heuristics. The dataset covers 44 languages ranging from low to high-resource, for many of which no public dataset is currently available. XL-Sum is highly abstractive, concise, and of high quality, as indicated by human and intrinsic evaluation. We fine-tune mT5, a state-of-the-art pretrained multilingual model, with XL-Sum and experiment on multilingual and low-resource summarization tasks. XL-Sum induces competitive results compared to the ones obtained using similar monolingual datasets: we show higher than 11 ROUGE-2 scores on 10 languages we benchmark on, with some of them exceeding 15, as obtained by multilingual training. Additionally, training on low-resource languages individually also provides competitive performance. To the best of our knowledge, XL-Sum is the largest abstractive summarization dataset in terms of the number of samples collected from a single source and the number of languages covered. We are releasing our dataset and models to encourage future research on multilingual abstractive summarization. The resources can be found at \url{https://github.com/csebuetnlp/xl-sum}.

==> backup.tex <==
\section{Introduction}

\begin{table}[h]
\centering
%\small
\begin{tabular}{p{\linewidth}}
\hline
\hline
\textbf{Input Article:} Antibodies are a key part of our immune defences and stop the virus from getting inside the body's cells. The Imperial College London team found the number of people testing positive for antibodies has fallen by 26\% between June and September. [...] \iffalse
They say immunity appears to be fading and there is a risk of catching the virus multiple times.

The news comes as figures from the Office for National Statistics show that the number of Covid-19 deaths in the UK rose by 60\% in the week of 16 October.

The ONS figures suggest there have now been more than 60,000 deaths involving Covid-19 in the UK.

More than 350,000 people in England have taken an antibody test as part of the REACT-2 study so far.

In the first round of testing, at the end of June and the beginning of July, about 60 in 1,000 people had detectable antibodies.

But in the latest set of tests, in September, only 44 per 1,000 people were positive.

It suggests the number of people with antibodies fell by more than a quarter between summer and autumn.\fi ``Immunity is waning quite rapidly, we're only three months after our first [round of tests] and we're already showing a 26\% decline in antibodies," said Prof Helen Ward, one of the researchers. [...] \iffalse
The fall was greater in those over 65, compared with younger age groups, and in those without symptoms compared with those with full-blown Covid-19.

The number of healthcare workers with antibodies remained relatively high, which the researchers suggest may be due to regular exposure to the virus.\fi Antibodies stick to the surface of the coronavirus to stop it invading our body's cells and attacking the rest of the immune system. [...] \iffalse Exactly what the antibody drop means for immunity is still uncertain. There are other parts of the immune system, such as T-cells, which may also play a role, directly killing infected host cells and calling to other immune cells to help out.

However, the researchers warn antibodies tend to be highly predictive of who is protected.

Prof Wendy Barclay said: "We can see the antibodies and we can see them declining and we know antibodies on their own are quite protective.

"On the balance of evidence, I would say it would look as if immunity declines away at the same rate as antibodies decline away, and that this is an indication of waning immunity."

There are four other seasonal human coronaviruses, which we catch multiple times in our lives. They cause common cold symptoms and we can be reinfected every six to 12 months.

Many people have mild or asymptomatic coronavirus infections.

Two out of every three people who tested positive for coronavirus in a study published today by the Office for National Statistics experienced none of the main symptoms of coronavirus.

Separate figures from the ONS today showed that Covid-19 deaths in the UK increased from just under 500 to just over 750 in the week to 16 October, pushing the total number of deaths 6\% over the level expected for this time of year.

The ONS figures suggest that more than 60,000 deaths in the UK have involved coronavirus so far this year.

By 16 October, more than 59,000 of these deaths had happened and, since then, a further 1,200 people have died within 28 days of a positive test for coronavirus. Ninety per cent of these deaths happened before the end of June.

There have been very few confirmed cases of people getting Covid twice. However, the researchers warn this may be due to immunity only just starting to fade since the peak infection rates of March and April.

The hope is the second infection will be milder than the first, even if immunity does decline, as the body should have an "immune memory" of the first encounter and know how to fight back.

The researchers say their findings do not scupper hopes of a vaccine, which may prove more effective than a real infection.
\fi One of the researchers, Prof Graham Cooke, said: ``The big picture is after the first wave, the great majority of the country didn't have evidence of protective immunity. [...]\\

\iffalse 
"The need for a vaccine is still very large, the data doesn't change that."

Professor Paul Elliott, director of the REACT-2 study, said it would be wrong to draw firm conclusions from the study about the impact of a vaccine.

He said: "The vaccine response may behave differently to the response to natural infection."

But he said it was possible that some people might need follow-up booster doses of any vaccine that became available to top up fading immunity over time.\fi
\hline
\hline
\textbf{Summary:} Levels of protective antibodies in people wane ``quite rapidly" after coronavirus infection, say researchers. \\
\hline
\hline
\end{tabular}
\caption{A sample article-summary pair, some portions of the input article have been truncated for brevity reasons. \yb{Move Table 1 to the page being discussed.} \msi{enlarge caption with relevant information}}
\label{tab:example}
\end{table}

Automatic text summarization \citep{nenkova2011automatic} is a fundamental problem in natural language processing. Given an input text (i.e., typically a long document or article), the goal is to generate a smaller, concise piece of text that conveys the key information of the input. There are two main approaches to automatic text summarization: \textit{extractive} and \textit{abstractive}. Extractive methods crop out one or more segments from the input text and concatenate them to produce a summary. \yb{Can we add what's the limit of the extractive approach}
Abstractive summarization, on the other hand, generates summaries that may contain words and phrases not present in the input text (e.g., via paraphrasing), and may arguably relate more to human genrated summaries. \yb{Can we add what's the advantage of the abstractive approach over extractive approach} Although abstractive summaries can be more coherent and concise than extractive summaries \citep{cohn2008sentence}, generating them is more challenging due to the nature of this task. The success of sequence-to-sequence (seq2seq) models \citep{cho2014learning, sutskever2014sequence} over the last decade has rejuvenated abstractive text summarization \citep{rush2015neural, see-etal-2017-get}, which had previously received much less attention in contrast to extractive approaches \citep{nenkova2012survey}. \yf{this expression is a bit `artistic', which is not a problem. However it can be made clearer in what it means. Does it mean extractive summarization has had better performance than abstractive summarization bofer seq2seq?}.

\begin{table*}[h]
\centering
\begin{tabular}{l}
\hline
\textbf{Language}\\
\hline
Oromo\\
Amharic\\
French\\
Hausa\\
Igbo\\
Gahuza\\
Pidgin\\
Somali\\
Swahili\\
Tigrinya\\
Yoruba\\
Kyrgyz\\
Uzbek\\
Burmese\\
Chinese (simplified)\\
Indonesian\\
Japanese\\
Korean\\
Thai\\
Vietnamese\\
Arabic\\
Persian\\
\hline
\\
\hline
\end{tabular}
\begin{tabular}{r}
\hline
\textbf{Article-Summary Pairs}\\
\hline
6,568\\
6,163\\
11,781\\
7,459\\
5,551\\
6,119\\
10,972\\
6,719\\
11,766\\
5,621\\
7,972\\
2,889\\
7,123\\
8,825\\
43,577\\
46,545\\
11,048\\
5,009\\
7,929\\
7,244\\
56,688\\
32,590\\
\hline
\textbf{Total}\\
\hline
\end{tabular}
\centering
\begin{tabular}{l}
\hline
\textbf{Language}\\
\hline
Bengali\\
Gujarati\\
Hindi\\
Marathi\\
Nepali\\
Pashto\\
Punjabi\\
Sinhala\\
Tamil\\
Telugu\\
Urdu\\
Azeri\\
English\\
Scottish Gaelic\\
Russian\\
Serbian (Cyrillic)\\
Serbian (Latin)\\
Turkish\\
Ukrainian\\
Welsh\\
Portuguese\\
Spanish\\
\hline
\textbf{1,132,024}\\
\hline
\end{tabular}
\begin{tabular}{r}
\hline
\textbf{Article-Summary Pairs}\\
\hline
10,118\\
10,610\\
61,204\\
12,238\\
6,119\\
21,642\\
10,341\\
8,548\\
19,593\\
12,310\\
51,441\\
9,219\\
303,136\\
1,094\\
60,297\\
8,913\\
8,851\\
31,328\\
64,312\\
12,256\\
26,450\\
46,563\\
\hline
\\
\hline
\end{tabular}
\label{tab:dataset}
\caption{Languages and Article-summary statistics of the XL-Sum dataset}\label{tab:data}
\end{table*}

Typical seq2seq-based models are heavily data-driven, i.e., a large number of article-summary pairs are required to train them effectively. As a result, abstractive summarization has centered around the English language, as most large abstractive summarization datasets \citep{hermann2015teaching, grusky2018newsroom, narayan2018don} are available in English only. Though there have been some recent efforts for curating multilingual abstractive summarization datasets \citep{giannakopoulos2015multiling, cao2020multisumm, scialom2020mlsum}, they are limited either in terms of the number of languages covered or the number of available training samples.


In this work, we introduce \textbf{XL-Sum}, a large-scale abstractive summarization dataset of news articles crawled from the British Broadcasting Corporation (BBC)\footnote{\url{https://www.bbc.com/}} website. Using a custom crawler, we collect more than 1 million professionally annotated article-summary pairs covering 44 languages. Originating from a single source, these samples exhibit similar summarization strategies across all languages, making them ideal for the multilingual summarization task. In addition to it, we also conduct experiments on low-resource and cross-lingual summarization tasks using pre-trained models and show \hl{up to 15 ROUGE-2 score} \yf{`score differences'?} on different languages. 
\yb{In abstract, we said 11 but here 15. Please doublecheck}
\yf{also, what does this result say about the dataset in terms of its diversity, significance, difficulty, etc.?}
\yf{`We will release the dataset, curation tools and summarization model checkpoints with this paper.'}
We believe that our efforts in this work will encourage the community to push the boundary of abstractive text summarization beyond the English language, especially for low and mid-resource languages. \iffalse \fi



\section{The XL-Sum Dataset}

In this section, we discuss the curation process of the XL-Sum dataset.
\yb{If you have a space, a figure showing the entire curation process would be valuable. And here, we can describe its overview - emphasising some of our unique directions for curation.}

\subsection{Content Source}

BBC publishes news in 43 languages\footnote{\url{https://www.bbc.co.uk/ws/languages}} ranging from low-resource languages like Bengali and Swahili to high-resource ones like English and Russian. Among the 43 languages, Serbian is a special case which is published using both Cyrillic, the official script, and also Latin, the colloquial script. We treat them as different languages in this work, totalling to a coverage of 44 languages.

\subsection{Content Search}

As BBC does not provide any archive or RSS feed on their website, we designed a custom crawler to recursively crawl pages starting from the homepage by visiting the different article links present in each page visited. \yf{(1) this is engineering work so it's not a research challenge, (2) it doesn't seem to be be a very challenging task since web crawling is a mature technology. I suggest we remove this sentence} The BBC websites for different languages have similar structures, so our crawler was able to scrape articles from all sites. Before proceeding to the next stage of the pipeline, we discarded pages with no text content (mostly constituting media pages). \yf{you mean text-only pages without any image, etc.? this seems overly restrictive}.

\subsection{Article-Summary Extraction}

Collecting automatic summaries of articles differs across different datasets. For example, the CNN/DM dataset \citep{hermann2015teaching} merged bullet point highlights provided with the articles as reference summaries, whilst the Xsum dataset \citep{narayan2018don} used the first line of the article as the summary and the rest of the article as the input.

Our method of collecting automatic summaries was made easier by the nature of the BBC articles we crawled. BBC typically provides a summary of a whole article in the form of a bold paragraph at the beginning of each article. These summaries are written professionally by the authors of the articles in order to convey the main story of the article within one small paragraph. We used the whole paragraph, generally containing one, and in some cases two sentences, as the summary while using the rest of the article as the input reference, and discarded the \hl{headline} \yf{title?} completely. (We show in Table \ref{tab:example} an example article-summary pair from BBC English.) \st{We designed an HTML parser to perform the extraction accordingly.} This strategy of automatic annotation of summaries resembles Xsum to some extent, but we found the first line to contain meta-information in many articles (e.g., author information, date of last modification). As such, we used the bold paragraphs as the summary instead.

\yb{Can we provide some examples showing what are inputs and outputs required for each curation step above?}

\yf{on Yong-Bin's suggestion, may want to show a screenshot of a web page and highlight the article and the summary}

Table \ref{tab:data} shows the article-summary statistics for all languages in the XL-Sum dataset. 

\section{Intrinsic Evaluation of XL-Sum}
\yb{Why we call "Intrinsic Evaluation". Can we explain about it further?}

At this point, a discussion is warranted about the extractiveness and quality of the XL-Sum dataset, since the article-summary pairs were collected automatically (albeit being written by professionals). We provide both human and automatic evaluations.

\yb{Suggestion: Evaluating the extractiveness and quality of the XL-Sum dataset is crucial to ensure that it can be valuable and used in wider community for abstractive summarization.  For this, we thoroughly conduct both human and automatic evaluations using the article-summary pairs were collected automatically (albeit being written by professionals).}

\yb{Human evaluation provides us with what insight? The same with automatic evaluation. Can we provide some benefits of each of these evaluations?}
\subsection{Human Evaluation}\label{sec:human}

We hired professional annotators\msi{-- minimum education level: undergraduate student, and minimum proficiency level: native speaker/ have advanced level of proficiency determined by professional language tests for the corresponding language. For the top-10 languages according to the number of speakers\footnote{\url{https://w.wiki/Pss}}, each annotator was asked to assess the quality of a random subset of the dataset (250 article-summary pairs) by answering the following questions with `Yes'/`No':}

\yb{We need to justify why these 3 properties can be enough to assess the quality of the dataset. Some references or rationale or hypothesis are needed.}

\begin{enumerate}
    \item \textbf{Property A:} Does the summary convey what the article is about?
    \item \textbf{Property B:} If the answer to property \verb!A! is `Yes', does the summary contain any information that in inconsistent the the article?
    \item \textbf{Property C:} If the answer to property \verb!A! is `Yes', does the summary contain any information that cannot be inferred from the article?
\end{enumerate}

The motivation for designing the properties stemmed from recent progresses on the quality estimation of neural language generation (NLG) models. \citet{belinkov2017synthetic} showed that NLG models are vulnerable to noisy and low-quality training samples, hence, it its essential to validate the quality of the summary through Property \verb!A!. Ensuring factual consistency and faithfulness \citep{wang2020asking, maynez2020faithfulness} of the generated summaries is also a key consideration for neural abstractive summarization, since neural models have been shown to generated hallucinated texts \citep{see-etal-2017-get}. Property \verb!B! checks for consistency between the article and summary; while Property \verb!C! assesses the hallucination implicitly by limiting the knowledge domain to the input article and identifying additional information in the summary.

It is desired that property \verb!A! would have a high percentage of `Yes', while property \verb!B! and \verb!C! would have a low percentage. The third property can be a bit ambiguous, since some pieces of information may be not directly be present in the input article, but a professional with some background knowledge and understanding of the article topic may infer them inherently. 

Since text summarization is posed as a closed domain task, we asked the annotators to label accordingly, to not make use of any addition information outside the article. We also provided them with some sample annotations in English to aid them during annotation. The percentage of the three properties are shown in Table \ref{tab:human}.

\begin{table}[h]
    \centering
    \begin{tabular}{l}
    \hline
    \textbf{Language}\\
    \hline
    1. English\\
    2. Chinese\\
    3. Hindi\\
    4. Spanish\\
    5. French\\
    6. Arabic\\
    7. Bengali\\
    8. Russian\\
    9. Portuguese\\
    10. Indonesian\\
    \hline
    \end{tabular}
    \begin{tabular}{ccc}
    \hline
    \textbf{A} & \textbf{B} & \textbf{C}\\
    \hline
    99.67 & x & x\\
    97.56 & x & x\\
    90.91 & x & x\\
    84.71 & x & x\\
    100 & x & x\\
    99.59 & x & x\\
    91.13 & x & x\\
    95.65 & x & x\\
    88.01 & x & x\\
    97.59 & x & x\\
    \hline
    \end{tabular}
    \caption{Human evaluation metrics of XL-Sum}\label{tab:human}
\end{table}

Most languages showed a high percentage of good summaries in the upper nineties, while some had a slightly lower percentage (i.e., Spanish and Portuguese). We were informed by the annotators that the negative summaries were mostly extracted from opinion pieces and blog posts the bold paragraphs of which did not convey the main story of the articles. 

Little to no good summaries had any conflicting information, while about half of the summaries had information that were not directly inferrable. Interestingly, more than 75\% of the latter had missing information like first names or abbreviations of acronyms. For example, a summary had the phrase `president-elect Joe Biden' while its corresponding article had no presence of the first name `Joe'. Another article had NHS abbreviated in  the summary, which was missing in the article. 

The presence of extra information in the summaries is understandable, since professional experts writing these summaries not only use the information present in the article text, but also imbue their knowledge and understanding of the outside world. But for a closed domain summarization model or a layman to this topic, inferring this information is not so straightforward, which makes the automated abstractive summarization task more challenging.
Perhaps, this explains why language models fine-tuned on pretrained checkpoints \citep{raffel2019exploring, yan2020prophetnet, zhang2020pegasus} are achieving state-of-the-art results in abstractive summarization, being able to make use of the information gained from the high volume of texts they were pretrained with. %This doesn't necessarily deteriorate the quality of the dataset, but rather makes abstractive summarization a more challenging task.For a person with knowledge of these topics, this is a trivial task; but for a closed domain summarization model or a layman to this topic, inferring this information is not so straightforward.  
\msi{Additionally, it would be interesting to see whether the recent trend of incorporating real-world knowledge and common sense reasoning ~\cite{tandon2018commonsense, deng2020integrating} into the machine learning models works out for text summarization.}

\subsection{Automatic Evaluation}

While the human evaluations gave us a quantitative insight into the the quality of XL-Sum for different languages, an evaluation of the abstractiveness is also needed. As such, we sampled 5000 articles from the 10 languages discussed in Section \ref{sec:human}. We show the percentage of novel n-grams ($n = 1, 2, 3, 4$) in the gold summary with respect to the input article in Table \ref{tab:ngram}. Before computing the n-grams to removed punctuation marks, and additionally for Chinese, we split the characters. We also show these metrics for Xsum using the same processing. 

\begin{table}[h]
    \centering
    \begin{tabular}{l}
    \hline
    \scriptsize{\textbf{LANGUAGE}}\\
    %\textbf{Language}\\
    \hline
    Xsum\\
    English\\
    Chinese\\
    Hindi\\
    Spanish\\
    French\\
    Arabic\\
    Bengali\\
    Russian\\
    Portuguese\\
    Indonesian\\
    \hline
    \end{tabular}
    \begin{tabular}{c @{\hspace{.1cm}} c @{\hspace{.1cm}} c @{\hspace{.1cm}} c}
    \hline
    \scriptsize{\textbf{UNIGRAM}} & \scriptsize{\textbf{BIGRAM}} & \scriptsize{\textbf{TRIGRAM}} & \scriptsize{\textbf{4-GRAM}}\\
    %\textbf{1} & \textbf{2} & \textbf{3} & \textbf{4}\\
    \hline
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    x & x & x & x\\
    \hline
    \end{tabular}
    \caption{Percentage of novel n-grams in gold summary}\label{tab:ngram}
    \end{table}

\section{Experiments and Results}

Initializing Transformer-based \citep{vaswani2017attention} seq2seq models with pre-trained weights from self-supervised training \citep{raffel2019exploring,  rothe2020leveraging, yan2020prophetnet} have been shown to achieve state-of-the-art results on abstractive text summarization. Even with only 3,000 training samples, \citet{khandelwal2019sample} managed to get non-trivial results \textcolor{orange}{with} a summarization model fine-tuned on the GPT-2 \citep{radford2019language} decoder. Thus, we followed the same approach for our experiments. There are many multilingual pre-trained checkpoints available through the Huggingface Transformers Library \citep{wolf2020transformers}. We chose to use the mT5 model \citep{xue2020mt5} for its support of a wide coverage of languages.  

For all languages, we randomly sampled $500$ pairs for \st{dev}\textcolor{orange}{the development} set and $500$ pairs for the test set. We tokenized our training samples using the 250k wordpiece \citep{wu2016google} vocabulary provided with the mT5 checkpoint.  Due to computational constraints, we had to truncate the inputs to $512$ tokens and the outputs to $64$ tokens. We used the ROUGE-1, ROUGE-2 and ROUGE-L \citep{lin2004rouge} scores for automatic evaluation. For inference, we used beam search with beam size $4$ and length penalty of $\alpha=0.6$ \citep{wu2016google}. We performed summarization experiments on three premises: (i) multilingual,  (ii) low-resource and (iii) cross-lingual setups.

\subsection{Multilingual Summarization}

Multilingual training has been used previously several NLP tasks like neural machine translation \citep{arivazhagan2019massively} and language model pretraining \citep{lample2019cross}. However, we found no relevant work that performed multilingual summarization. 

For the multilingual experiment, we followed a similar training setup as \citep{lample2019cross}: We sampled each batch from a single language containing 256 samples and used a smoothing factor ($\alpha$) of 0.5 such that low-resource languages would be sampled at a higher rate such that they don't underfit. We trained the model for 35k steps with the Adafactor optimization algorithm \citep{shazeer2018adafactor} with a linear warmup of 5000 steps and square root decay of the learning rate. We show the ROUGE scores of the model on the top 10 languages discussed in section \ref{sec:human} in Table \ref{tab:mult}.

\begin{table}[h]
\centering
\begin{tabular}{l}
\hline
\textbf{Language}\\
\hline
English\\
Chinese\\
Hindi\\
Spanish\\
French\\
Arabic\\
Bengali\\
Russian\\
Portuguese\\
Indonesian\\
\hline
\end{tabular}
\begin{tabular}{c}
\hline
\textbf{R-1 / R-2 / R-L}\\
\hline
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
??? / ??? / ???\\
\hline
\end{tabular}
\caption{ROUGE scores for multilingual summarization}\label{tab:mult}
\end{table}

\textcolor{red}{Add discussions after getting the results.}

\subsection{Low-Resource Summarization}

Languages having less than $15,000$ training pairs may be treated as low-resource language for our experiments. Several low-resource languages are present in our dataset. Among them, we choose Bengali and Swahili for our experiments. For these experiments, we used a batch size of 32 and trained for 10 epochs with a slanted learning rate schedule \citep{howard2018universal}. We show the ROUGE scores in Table \ref{tab:low}.

\begin{table}[h]
\centering
\begin{tabular}{l}
\hline
\textbf{Language}\\
\hline
Bengali\\
Swahili\\
\hline
\end{tabular}
\begin{tabular}{c}
\hline
\textbf{R-1 / R-2 / R-L}\\
\hline
??? / ??? / ???\\ 
??? / ??? / ???\\ 
\hline
\end{tabular}
\caption{ROUGE scores for low-resource summarization}\label{tab:low}
\end{table}

\textcolor{red}{Add discussions after getting the results.}

\subsection{Cross-Lingual Summarization}

Cross lingual summarization \citep{zhu2019ncls} is done by training on one language and evaluating on another language. We chose two pairs of languages for cross-lingual experiment: one similar language pair, Hindi-Nepali another distant language pair, Portuguese-Russian, to see how the models were able to transfer across both distant and similar language pairs. ROUGE scores for distant and similar language pairs are shown is Table \ref{tab:similar} and Table \ref{tab:distant} respectively. The languages on the first column indicate the languages the respective model was trained on and the languages on the first row indicate the languages they were evaluated on.


\begin{table}[h]
\centering
\begin{tabular}{l}
\hline
\textbf{Language}\\
\hline
Hindi\\
Nepali\\
\hline
\end{tabular}
\begin{tabular}{cc}
\hline
Hindi & Nepali\\
\hline
???/???/??? & ???/???/???\\ 
???/???/??? & ???/???/???\\ 
\hline
\end{tabular}
\caption{ROUGE scores for cross-lingual summarization on similar language pairs}\label{tab:similar}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l}
\hline
\textbf{Language}\\
\hline
Portuguese\\
Russian\\
\hline
\end{tabular}
\begin{tabular}{cc}
\hline
Portuguese & Russian\\
\hline
???/???/??? & ???/???/???\\ 
???/???/??? & ???/???/???\\ 
\hline
\end{tabular}
\caption{ROUGE scores for cross-lingual summarization on distant language pairs}\label{tab:distant}
\end{table}

\textcolor{red}{Add discussions after getting the results.}

\section{Related Works}
\citet{rush2015neural} devised the first line of attack towards neural abstractive summarization using attentional seq2seq models \citep{bahdanau2014neural}. \citet{see-etal-2017-get} introduced pointer generator networks for abstractive summarization, that can learn to copy words from the input text, in addition to generating new texts with the decoder. \citet{narayan2018don} proposed a topic-aware convolutional seq2seq model for abstractive summarization. 

\citet{liu2019text} initialized the encoder and \citet{rothe2020leveraging} initialized both encoder and decoder of a seq2seq model with pre-trained BERT \citep{devlin2018bert} encoder  and fine-tuned the models for abstracitve summarization. \citet{raffel2019exploring, yan2020prophetnet} used fully pre-trained seq2seq models, while \citet{zhang2020pegasus} introduced a summarization-specific pre-training objective to achieve state-of-the-art results on multiple datasets. 

Most works on abstractive summarization have so far been limited to English, because of the lack of benchmark datasets for other languages. \citet{giannakopoulos2015multiling} introduced Multiling 2015, a summarization dataset spanning $40$ language, but the training set had only $10K$ samples in total. \citet{cao2020multisumm, scialom2020mlsum} introduced two new datasets for multilingual summarization, but they were limited to less than $10$ languages. Moreover, samples for different languages were collected from different sources, making them exposed to different types of summarization strategies, questioning the uniformity of the summaries.
